Streaming quanta sensors for online, high-performance imaging and vision

Recently quanta image sensors (QIS) -- ultra-fast, zero-read-noise binary image sensors -- have demonstrated remarkable imaging capabilities in many challenging scenarios. Despite their potential, the adoption of these sensors is severely hampered by (a) high data rates and (b) the need for new computational pipelines to handle the unconventional raw data. We introduce a simple, low-bandwidth computational pipeline to address these challenges. Our approach is based on a novel streaming representation with a small memory footprint, efficiently capturing intensity information at multiple temporal scales. Updating the representation requires only 16 floating-point operations/pixel, which can be efficiently computed online at the native frame rate of the binary frames. We use a neural network operating on this representation to reconstruct videos in real-time (10-30 fps). We illustrate why such representation is well-suited for these emerging sensors, and how it offers low latency and high frame rate while retaining flexibility for downstream computer vision. Our approach results in significant data bandwidth reductions ~100X and real-time image reconstruction and computer vision -- $10^4$-$10^5$ reduction in computation than existing state-of-the-art approach while maintaining comparable quality. To the best of our knowledge, our approach is the first to achieve online, real-time image reconstruction on QIS.

==> 01_introduction.tex <==
\section{Introduction}

\IEEEPARstart{U}{ltra-fast} binary quanta image sensors (QIS) have demonstrated novel imaging capabilities in challenging environments, including high dynamic range imaging, ultra-low light imaging, and high-speed imaging \cite{ma2020quanta}\cite{fossum2016quanta}\cite{ingle2019high}. This makes them attractive for a wide range of applications such as autonomous driving, robotics, remote sensing, and bio-imaging, where low light, large brightness changes, and/or fast motion are prevalent.

QIS sensors work by coupling single photon detectors with ultra-fast frame readout circuits. SPAD-QIS, a prominent QIS implementation \cite{ulku2018512}\cite{duttonSPADbasedQVGA2016}, can output binary frames free of read noise at speeds reaching up to 100~kFPS. The binary data streams generated by these sensors contain rich, fine-grained temporal information. Recent works have shown that when given access to all the binary data, it is possible to align and fuse the binary frames to output clean and sharp image/video reconstructions, allowing us to resolve high-speed details, even under low light levels and high dynamic range \cite{ma2020quanta}\cite{chandramouliBitToo2019}.

\textbf{Challenges of quanta sensing:} While quanta sensors are gradually becoming more readily available, there are several critical challenges that need to be addressed before they can be deployed in real-world applications. 
The first challenge is the \textit{huge data bandwidth} needed to stream the raw binary frames off the sensor. 
A QIS of 1~megapixel operating at 100~kFPS produces data at a rate of 100~Gbps---an impractically high-bandwidth data stream. This large bandwidth also results in prohibitive power and memory requirements. The second problem is the large computational cost involved with processing all the binary frames to produce quality images or perform downstream inferences. This problem is exacerbated by the unconventional nature of raw sensor data (a binary, quantized, and noisy bit-stream), which necessitates additional pre-processing steps before traditional computer vision algorithms can be applied. Recent pre-processing algorithms \cite{ma2020quanta} require several minutes of processing per second of input data---a computational cost that is four to five orders of magnitude slower than real-time. In spite of the promise of quanta image sensors, these practical challenges are inhibiting the deployment of this promising technology in resource-constrained applications that need to operate in real time.

We propose data structures, computational architectures, and associated algorithms that together address these challenges and close the gap towards near-real-time operation with QIS sensors. First, we propose a compact streaming representation that has a low memory footprint, can be updated in real-time with low compute complexity (a small number of additions and multiplications per pixel update), and stores rich information about the scene texture and motion at multiple temporal resolutions. We couple this representation with a feed-forward neural network to yield image reconstruction and high-level inference in real time (Fig.~\ref{fig:teaser}), with quality comparable to existing, resource-intensive approaches \cite{ma2020quanta}. Together, this representation and a feed-forward reconstruction algorithm yield near-real-time performance (Fig.~\ref{fig:teaser}), with a significant reduction in data bandwidth.

\textbf{Streaming representations:} The proposed streaming representations are updated when every new QIS frame arrives, thus minimizing the latency between the occurrence of a change and its capture. These high-speed updates are only possible due to the lack of read noise in SPAD-QIS; in a conventional sensor, sampling the scene at an equivalent rate would result in unacceptably high read noise.

Our streaming representation maintains information at multiple temporal scales, thereby encoding information about objects moving at varying speeds. Downstream inference algorithms (e.g., image reconstruction, face tracking, object detection) can \textit{poll} the representation at an arbitrary rate, based on the application needs and the computational resources available. Our representation allows us to build a seamless interface between a $\approx$100~kFPS sensor and $\approx$100~FPS vision algorithms, without incurring a latency penalty.

\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/fig_teaser_v2.pdf}
    \caption{\textbf{Top:} We propose a novel online processing architecture for QIS, which consists of streaming an extreme multi-exposure stack, and a modified U-Net with ResNet blocks for performing the reconstruction. The approach results in good image reconstruction performance. \textbf{Bottom:} The exposure stack is computed via a streaming update (figure bottom). Such a representation ensures information up to the most recent time instant is always available and decouples exposure from frame-read out. The sensor produces a consistent and continuously updated multi-exposure stack for any downstream request with near-zero lag.}
    \label{fig:teaser}
\end{figure*}

\textbf{Contributions:}
In summary, our proposed pipeline enables high-speed streaming vision with QIS sensors by combining a compact, streaming representation with a feed-forward neural network. The main contributions of the paper are:
\begin{itemize}
    \item A novel online representation and corresponding processing algorithms for quanta image sensors that are suitable for real-time systems.
    This representation lowers the bandwidth requirements by approximately two orders of magnitude (relative to reading out raw bitplanes), to a level compatible with current processing pipelines and data transfer interfaces.
    This representation can be continuously updated with just 16 floating point operations per pixel per binary frame, resulting in low latency and high computational efficiency.
    \item We design a feed-forward neural network for image reconstruction that denoises, aligns and integrates the multi-exposure representation into a clean intensity frame. The network is compact and can run in real-time on a desktop GPU (tens of FPS), resulting in an 4-5 orders of magnitude speed-up compared to existing methods for image reconstruction from quanta sensors. 
    \item We provide a rich, semi-realistic dataset that combines data from real cameras with 3D-simulated data. This dataset can be used for supervised learning on dynamic QIS problems. It contains diverse object categories and motion statistics. It generalizes across light levels, and can realistically represent camera captures of the 3D world.
    \item We demonstrate the application of our representation, architecture, and algorithms to several traditional computer vision tasks such as face detection, object detection, human pose estimation, and tracking. We demonstrate for the first time that such computer vision tasks can be applied to QIS data with near-real-time performance. 
\end{itemize}

